HarmonicNeRF: Geometry-Informed Synthetic View Augmentation for 3D Scene Reconstruction in Driving Scenarios

In the realm of autonomous driving, achieving precise 3D reconstruction of the driving environment is critical for ensuring safety and effective navigation. Neural Radiance Fields (NeRF) have shown promise in creating highly detailed and accurate models of complex environments. However, the application of NeRF in autonomous driving scenarios encounters several challenges, primarily due to the sparsity of viewpoints inherent in camera trajectories and the constraints on data collection in unbounded outdoor scenes, which typically occur along predetermined paths. This limitation not only reduces the available scene information but also poses significant challenges for NeRF training, as the sparse and path-distributed observational data leads to under-representation of the scene's geometry. In this paper, we introduce HarmonicNeRF, a novel approach for outdoor self-supervised monocular scene reconstruction. HarmonicNeRF capitalizes on the strengths of NeRF and enhances surface reconstruction accuracy by augmenting the input space with geometry-informed synthetic views. This is achieved through the application of spherical harmonics to generate novel radiance values, taking into careful consideration the color observations from the limited available real-world views. Additionally, our method incorporates proxy geometry to effectively manage occlusion, generating radiance pseudo-labels that circumvent the limitations of traditional image-warping techniques, which often fail in sparse data conditions typical of autonomous driving environments. Extensive experiments conducted on the KITTI, Argoverse, and NuScenes datasets demonstrate our approach establishes new benchmarks in synthesizing novel depth views and reconstructing scenes, significantly outperforming existing methods. Project page: https://github.com/Jiawei-Yao0812/HarmonicNeRF

==> figures/depth.tex <==

\begin{figure}[!b]
    \centering
    \rotatebox[origin=C]{90}{\parbox{20mm}{\centering \small NeuS }} 
  \mpage{0.18}{\includegraphics[width=\linewidth]{figures/figure_source/depth/depth_gt.jpg}}
  \mpage{0.18}{\includegraphics[width=\linewidth]{figures/figure_source/depth/depth_img_neus.jpg}}
  \mpage{0.18}{\includegraphics[width=\linewidth]{figures/figure_source/depth/depth_depth_neus.jpg}}
  \mpage{0.18}{\includegraphics[width=\linewidth]{figures/figure_source/depth/depth_mask_neus.jpg}}
  \\
  \rotatebox[origin=C]{90}{\parbox{20mm}{\centering \small Ours}} 
  \mpage{0.18}{\includegraphics[width=\linewidth]{figures/figure_source/depth/depth_gt.jpg}}
  \mpage{0.18}{\includegraphics[width=\linewidth]{figures/figure_source/depth/depth_img_ours.jpg}}
  \mpage{0.18}{\includegraphics[width=\linewidth]{figures/figure_source/depth/depth_depth_ours.jpg}}
  \mpage{0.18}{\includegraphics[width=\linewidth]{figures/figure_source/depth/depth_mask_ours.jpg}}
  \\
  \mpage{0.05}{\ }
  \mpage{0.175}{Ground Truth}
  \mpage{0.175}{Reconstructed View}
  \mpage{0.175}{Depth}
  \mpage{0.175}{Foreground Mask}
  \caption{Qualitative comparison of the reconstructed depth and foreground mask. The upper row is the result without novel radiance prediction. The lower row is the result using our method.}
  \label{fig:depth}
\end{figure}

==> figures/dtu_compare.tex <==
\begin{figure}[!b]
    \centering
    \vspace{-0.3cm}
    \rotatebox[origin=C]{90}{\parbox{20mm}{\centering \small Scan 40 \\ (DTU)}} 
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene40_47_gt.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene40_47_sparse.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene40_47_mvs1.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene40_47_sparse.jpeg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene40_47_ours.jpg}}
  \\
  \rotatebox[origin=C]{90}{\parbox{20mm}{\centering \small Scan 114 \\ (DTU)}} 
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene114_47_gt.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene114_47_NeuS.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene114_47_mvs.jpeg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene114_47_sparse.jpeg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/scene114_47_ours.jpg}}
 \\
   \rotatebox[origin=C]{90}{\parbox{20mm}{\centering \small Chair \\ (Blender)}} 
 \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/chair_gt.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/chair_NeuS.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/chair_mvs.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/chair_sparse.jpeg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/chair_ours.jpg}}
 \\
   \rotatebox[origin=C]{90}{\parbox{20mm}{\centering \small Drums \\ (Blender)}} 
 \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/drum_gt.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/drum_NeuS.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/drum_mvs.jpg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/drum_sparse.jpeg}}
  \mpage{0.15}{\includegraphics[width=\linewidth]{figures/figure_source/compare_dtu/drum_ours.jpg}}
  \\
  \mpage{0.05}{\ }
  \mpage{0.15}{Ground Truth}
  \mpage{0.15}{NeuS}
  \mpage{0.15}{MVSNeRF}
  \mpage{0.15}{SparseNeuS}
  \mpage{0.15}{Ours}
  \caption{Qualitative results of novel view synthesis on DTU dataset~\cite{DTU} and Blender dataset~\cite{mildenhall2021nerf}. We train the model using 30\% images for real scenes in DTU dataset, and 6\% for synthetic scenes in Blender dataset. }
  \label{fig:nvs}
\end{figure}

==> figures/limitation.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{figures/limitation_123.pdf}
    \caption{Unsuccessful cases in our reconstruction. We can see that the mesh at the back of the objects have several rough regions because of lack of supervision.}
    \label{fig:limitation}
\end{wrapfigure}

==> figures/mesh.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/mesh.pdf}
    \caption{Qualitative result of mesh reconstruction on DTU dataset. The model is trained using 30\% of the images. }
    \label{fig:mesh}
\end{figure*}

==> figures/vis_check.tex <==
\vspace{-0.2cm}
\begin{table}[htbp]
    \centering
    \resizebox{\linewidth}{!}{
   % \begin{threeparttable}
        \begin{tabular}{c||c||c}
            \multicolumn{1}{c||}{}&\multicolumn{1}{c||}{}&\multicolumn{1}{c}{} \\
            \hline
            ScanID & \textbf{w/o} vis check & \textbf{w/} vis check \\
            \hline
            scan24 & 12.00 & 15.92 \\
            scan37 & 12.74 & 13.87 \\
            scan40 & 11.16 & 15.67 \\
            scan55 & 13.52 & 17.10 \\
            scan63 & 14.94 & 23.35 \\
            scan65 & 14.10 & 19.52 \\
            scan69 & 12.55 & 14.94 \\
            scan83 & 18.75 & 24.10 \\
            scan97 & 13.02 & 17.55 \\
            scan106 & 11.62 & 13.62 \\
            scan114 & 13.77 & 18.52 \\
            scan118 & 14.86 & 19.57 \\
            scan122 & 14.99 & 18.57 \\


            \hline
            mean & 13.69 & \textbf{17.87} \\

        \end{tabular}
    
  %  \end{threeparttable}
    }
    \caption{Ablation Study for the effectiveness of the visibility check. We compare the view synthesis results of enabling visibility and disabling visibility when reconstructing 13 scenes from DTU dataset~\cite{DTU} using 3 or 5 images for each scene. }
    \vspace{-0.6cm}
    \label{tbl:evaluate_comparision}

\end{table}

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


